Jets from a stellar-mass black hole are as relativistic as those from supermassive black holes

Relativistic jets from supermassive black holes in active galactic nuclei are amongst the most powerful phenomena in the universe, acting to regulate the growth of massive galaxies. Similar jets from stellar-mass black holes offer a chance to study the same phenomena on accessible observation time scales. However, such comparative studies across black hole masses and time scales remain hampered by the long-standing perception that stellar-mass black hole jets are in a less relativistic regime. We used radio interferometry observations to monitor the Galactic black hole X-ray binary 4U 1543-47 and discovered two distinct, relativistic ejections launched during a single outburst. Our measurements reveal a likely Lorentz factor of $\sim$ 8 and a minimum of 4.6 at launch with 95% confidence, demonstrating that stellar-mass black holes in X-ray binaries can launch jets as relativistic as those seen in active galactic nuclei.

==> test2.tex <==
\begin{thebibliography}{10}
\setcounter{enumiv}{40}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{2017ApJ...846...98J}
\bibinfo{author}{{Jorstad}, S.~G.} \emph{et~al.}
\newblock \bibinfo{title}{{Kinematics of Parsec-scale Jets of Gamma-Ray Blazars
  at 43 GHz within the VLBA-BU-BLAZAR Program}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{846}},
  \bibinfo{pages}{98} (\bibinfo{year}{2017}).

\bibitem{2019ApJ...874...43L}
\bibinfo{author}{{Lister}, M.~L.} \emph{et~al.}
\newblock \bibinfo{title}{{MOJAVE. XVII. Jet Kinematics and Parent Population
  Properties of Relativistically Beamed Radio-loud Blazars}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{874}},
  \bibinfo{pages}{43} (\bibinfo{year}{2019}).

\bibitem{2019ARA&A..57..467B}
\bibinfo{author}{{Blandford}, R.}, \bibinfo{author}{{Meier}, D.} \&
  \bibinfo{author}{{Readhead}, A.}
\newblock \bibinfo{title}{{Relativistic Jets from Active Galactic Nuclei}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{57}},
  \bibinfo{pages}{467--509} (\bibinfo{year}{2019}).

\bibitem{1992Natur.358..215M}
\bibinfo{author}{{Mirabel}, I.~F.}, \bibinfo{author}{{Rodriguez}, L.~F.},
  \bibinfo{author}{{Cordier}, B.}, \bibinfo{author}{{Paul}, J.} \&
  \bibinfo{author}{{Lebrun}, F.}
\newblock \bibinfo{title}{{A double-sided radio jet from the compact Galactic
  Centre annihilator 1E1740.7-2942}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{358}},
  \bibinfo{pages}{215--217} (\bibinfo{year}{1992}).

\bibitem{2004ARA&A..42..317F}
\bibinfo{author}{{Fender}, R.} \& \bibinfo{author}{{Belloni}, T.}
\newblock \bibinfo{title}{{GRS 1915+105 and the Disc-Jet Coupling in Accreting
  Black Hole Systems}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{42}},
  \bibinfo{pages}{317--364} (\bibinfo{year}{2004}).

\bibitem{1972_ApJ}
\bibinfo{author}{{Matilsky}, T.~A.}, \bibinfo{author}{{Giacconi}, R.},
  \bibinfo{author}{{Gursky}, H.}, \bibinfo{author}{{Kellogg}, E.~M.} \&
  \bibinfo{author}{{Tananbaum}, H.~D.}
\newblock \bibinfo{title}{{A New Transient Source Observed by UHURU}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{174}},
  \bibinfo{pages}{L53--L55} (\bibinfo{year}{1972}).

\bibitem{1984_PASJ}
\bibinfo{author}{{Kitamoto}, S.}, \bibinfo{author}{{Miyamoto}, S.},
  \bibinfo{author}{{Tsunemi}, H.}, \bibinfo{author}{{Makishima}, K.} \&
  \bibinfo{author}{{Nakagawa}, M.}
\newblock \bibinfo{title}{{The transient X-ray source 4U 1543-47 observed from
  Tenma.}}
\newblock \emph{\bibinfo{journal}{\pasj}} \textbf{\bibinfo{volume}{36}},
  \bibinfo{pages}{799--806} (\bibinfo{year}{1984}).

\bibitem{1992_IAUC}
\bibinfo{author}{{Harmon}, B.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{U 1543-47}}.
\newblock \emph{\bibinfo{journal}{\iaucirc}} \textbf{\bibinfo{volume}{5510}},
  \bibinfo{pages}{2} (\bibinfo{year}{1992}).

\bibitem{2002_IAUC}
\bibinfo{author}{{Miller}, J.~M.} \& \bibinfo{author}{{Remillard}, R.~A.}
\newblock \bibinfo{title}{{4U 1543-47}}.
\newblock \emph{\bibinfo{journal}{\iaucirc}} \textbf{\bibinfo{volume}{7920}},
  \bibinfo{pages}{2} (\bibinfo{year}{2002}).

\bibitem{2003_IAUS_Orosz}
\bibinfo{author}{{Orosz}, J.~A.}
\newblock \bibinfo{title}{{Inventory of black hole binaries}}.
\newblock In \emph{\bibinfo{booktitle}{A Massive Star Odyssey: From Main
  Sequence to Supernova}}, vol. \bibinfo{volume}{212}, \bibinfo{pages}{365}
  (\bibinfo{year}{2003}).
\newblock \eprint{astro-ph/0209041}.

\bibitem{2002_AAS_Orosz}
\bibinfo{author}{{Orosz}, J.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{Revised parameters for the black hole binary 4U
  1543-47}}.
\newblock In \emph{\bibinfo{booktitle}{American Astronomical Society Meeting
  Abstracts}}, vol. \bibinfo{volume}{201} of \emph{\bibinfo{series}{American
  Astronomical Society Meeting Abstracts}}, \bibinfo{pages}{15.11}
  (\bibinfo{year}{2002}).

\bibitem{2003_A&A_Ritter}
\bibinfo{author}{{Ritter}, H.} \& \bibinfo{author}{{Kolb}, U.}
\newblock \bibinfo{title}{{Catalogue of cataclysmic binaries, low-mass X-ray
  binaries and related objects (Seventh edition)}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{404}},
  \bibinfo{pages}{301--303} (\bibinfo{year}{2003}).

\bibitem{2023ApJ...946...19D}
\bibinfo{author}{{Draghis}, P.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{A Systematic View of Ten New Black Hole Spins}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{946}},
  \bibinfo{pages}{19} (\bibinfo{year}{2023}).

\bibitem{2020MNRAS.493.4409D}
\bibinfo{author}{{Dong}, Y.}, \bibinfo{author}{{Garc{\'\i}a}, J.~A.},
  \bibinfo{author}{{Steiner}, J.~F.} \& \bibinfo{author}{{Gou}, L.}
\newblock \bibinfo{title}{{The spin measurement of the black hole in 4U 1543-47
  constrained with the X-ray reflected emission}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{493}},
  \bibinfo{pages}{4409--4417} (\bibinfo{year}{2020}).

\bibitem{2006ApJ...636L.113S}
\bibinfo{author}{{Shafee}, R.} \emph{et~al.}
\newblock \bibinfo{title}{{Estimating the Spin of Stellar-Mass Black Holes by
  Spectral Fitting of the X-Ray Continuum}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{636}},
  \bibinfo{pages}{L113--L116} (\bibinfo{year}{2006}).

\bibitem{2009PASJ}
\bibinfo{author}{{Matsuoka}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{The MAXI Mission on the ISS: Science and Instruments
  for Monitoring All-Sky X-Ray Images}}.
\newblock \emph{\bibinfo{journal}{\pasj}} \textbf{\bibinfo{volume}{61}},
  \bibinfo{pages}{999} (\bibinfo{year}{2009}).

\bibitem{2009IEEEP_Jonas}
\bibinfo{author}{{Jonas}, J.~L.}
\newblock \bibinfo{title}{{MeerKAT - The South African Array With Composite
  Dishes and Wide-Band Single Pixel Feeds}}.
\newblock \emph{\bibinfo{journal}{IEEE Proceedings}}
  \textbf{\bibinfo{volume}{97}}, \bibinfo{pages}{1522--1530}
  (\bibinfo{year}{2009}).

\bibitem{fender2017thunderkat}
\bibinfo{author}{Fender, R.} \emph{et~al.}
\newblock \bibinfo{title}{Thunderkat: The meerkat large survey project for
  image-plane radio transients} (\bibinfo{year}{2017}).
\newblock \eprint{1711.04132}.

\bibitem{2004ApJ_Gehrels}
\bibinfo{author}{{Gehrels}, N.} \emph{et~al.}
\newblock \bibinfo{title}{{The Swift Gamma-Ray Burst Mission}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{611}},
  \bibinfo{pages}{1005--1020} (\bibinfo{year}{2004}).

\bibitem{2004MNRAS.355.1105F}
\bibinfo{author}{{Fender}, R.~P.}, \bibinfo{author}{{Belloni}, T.~M.} \&
  \bibinfo{author}{{Gallo}, E.}
\newblock \bibinfo{title}{{Towards a unified model for black hole X-ray binary
  jets}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{355}},
  \bibinfo{pages}{1105--1118} (\bibinfo{year}{2004}).

\bibitem{2004MNRAS.347L..52G}
\bibinfo{author}{{Gallo}, E.}, \bibinfo{author}{{Corbel}, S.},
  \bibinfo{author}{{Fender}, R.~P.}, \bibinfo{author}{{Maccarone}, T.~J.} \&
  \bibinfo{author}{{Tzioumis}, A.~K.}
\newblock \bibinfo{title}{{A transient large-scale relativistic radio jet from
  GX 339-4}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{347}},
  \bibinfo{pages}{L52--L56} (\bibinfo{year}{2004}).

\bibitem{2022ApJS..260...12W}
\bibinfo{author}{{Weaver}, Z.~R.} \emph{et~al.}
\newblock \bibinfo{title}{{Kinematics of Parsec-scale Jets of Gamma-Ray Blazars
  at 43 GHz during 10 yr of the VLBA-BU-BLAZAR Program}}.
\newblock \emph{\bibinfo{journal}{\apjs}} \textbf{\bibinfo{volume}{260}},
  \bibinfo{pages}{12} (\bibinfo{year}{2022}).

\bibitem{2002ApJ...569..362S}
\bibinfo{author}{{Smith}, D.~M.}, \bibinfo{author}{{Heindl}, W.~A.} \&
  \bibinfo{author}{{Swank}, J.~H.}
\newblock \bibinfo{title}{{Two Different Long-Term Behaviors in Black Hole
  Candidates: Evidence for Two Accretion Flows?}}
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{569}},
  \bibinfo{pages}{362--380} (\bibinfo{year}{2002}).

\bibitem{2004ApJ...611L.121Y}
\bibinfo{author}{{Yu}, W.}, \bibinfo{author}{{van der Klis}, M.} \&
  \bibinfo{author}{{Fender}, R.}
\newblock \bibinfo{title}{{The Correlation between Hard X-Ray Peak Flux and
  Soft X-Ray Peak Flux in the Outburst Rise of Low-Mass X-Ray Binaries}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{611}},
  \bibinfo{pages}{L121--L124} (\bibinfo{year}{2004}).

\bibitem{2007ApJ...663.1309Y}
\bibinfo{author}{{Yu}, W.}, \bibinfo{author}{{Lamb}, F.~K.},
  \bibinfo{author}{{Fender}, R.} \& \bibinfo{author}{{van der Klis}, M.}
\newblock \bibinfo{title}{{Peak Luminosities of the Hard States of GX 339-4:
  Implications for the Accretion Geometry, Disk Mass, and Black Hole Mass}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{663}},
  \bibinfo{pages}{1309--1314} (\bibinfo{year}{2007}).

\bibitem{2007A&A_Evans}
\bibinfo{author}{{Evans}, P.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{An online repository of Swift/XRT light curves of
  {\ensuremath{\gamma}}-ray bursts}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{469}},
  \bibinfo{pages}{379--385} (\bibinfo{year}{2007}).

\bibitem{2009MNRAS_Evans}
\bibinfo{author}{{Evans}, P.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{Methods and results of an automatic analysis of a
  complete sample of Swift-XRT observations of GRBs}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{397}},
  \bibinfo{pages}{1177--1201} (\bibinfo{year}{2009}).

\bibitem{1996ASPC_Arnaud}
\bibinfo{author}{{Arnaud}, K.~A.}
\newblock \bibinfo{title}{{XSPEC: The First Ten Years}}.
\newblock In \bibinfo{editor}{{Jacoby}, G.~H.} \& \bibinfo{editor}{{Barnes},
  J.} (eds.) \emph{\bibinfo{booktitle}{Astronomical Data Analysis Software and
  Systems V}}, vol. \bibinfo{volume}{101} of
  \emph{\bibinfo{series}{Astronomical Society of the Pacific Conference
  Series}}, \bibinfo{pages}{17} (\bibinfo{year}{1996}).

\bibitem{2016A&A_HI4PI}
\bibinfo{author}{{HI4PI Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{HI4PI: A full-sky H I survey based on EBHIS and
  GASS}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{594}},
  \bibinfo{pages}{A116} (\bibinfo{year}{2016}).

\bibitem{Remillard_2022}
\bibinfo{author}{Remillard, R.~A.} \emph{et~al.}
\newblock \bibinfo{title}{An empirical background model for the {NICER} x-ray
  timing instrument}.
\newblock \emph{\bibinfo{journal}{The Astronomical Journal}}
  \textbf{\bibinfo{volume}{163}}, \bibinfo{pages}{130} (\bibinfo{year}{2022}).
\newblock \urlprefix\url{https://doi.org/10.3847%2F1538-3881%2Fac4ae6}.

\bibitem{2007ASPC_McMullin}
\bibinfo{author}{{McMullin}, J.~P.}, \bibinfo{author}{{Waters}, B.},
  \bibinfo{author}{{Schiebel}, D.}, \bibinfo{author}{{Young}, W.} \&
  \bibinfo{author}{{Golap}, K.}
\newblock \bibinfo{title}{{CASA Architecture and Applications}}.
\newblock In \bibinfo{editor}{{Shaw}, R.~A.}, \bibinfo{editor}{{Hill}, F.} \&
  \bibinfo{editor}{{Bell}, D.~J.} (eds.) \emph{\bibinfo{booktitle}{Astronomical
  Data Analysis Software and Systems XVI}}, vol. \bibinfo{volume}{376} of
  \emph{\bibinfo{series}{Astronomical Society of the Pacific Conference
  Series}}, \bibinfo{pages}{127} (\bibinfo{year}{2007}).

\bibitem{2020ascl.soft_oxkat}
\bibinfo{author}{{Heywood}, I.}
\newblock \bibinfo{title}{{oxkat: Semi-automated imaging of MeerKAT
  observations}}.
\newblock \bibinfo{howpublished}{Astrophysics Source Code Library, record
  ascl:2009.003} (\bibinfo{year}{2020}).
\newblock \eprint{2009.003}.

\bibitem{1995PhDT.......238B}
\bibinfo{author}{{Briggs}, D.~S.}
\newblock \emph{\bibinfo{title}{{High fidelity deconvolution of moderately
  resolved sources}}}.
\newblock Ph.D. thesis, \bibinfo{school}{New Mexico Institute of Mining and
  Technology} (\bibinfo{year}{1995}).

\bibitem{2010MNRAS.402.2403M}
\bibinfo{author}{{Murphy}, T.} \emph{et~al.}
\newblock \bibinfo{title}{{The Australia Telescope 20 GHz Survey: the source
  catalogue}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{402}},
  \bibinfo{pages}{2403--2423} (\bibinfo{year}{2010}).

\bibitem{2016ApJ...821...61P}
\bibinfo{author}{{Partridge}, B.} \emph{et~al.}
\newblock \bibinfo{title}{{Absolute Calibration of the Radio Astronomy Flux
  Density Scale at 22 to 43 GHz Using Planck}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{821}},
  \bibinfo{pages}{61} (\bibinfo{year}{2016}).

\bibitem{2018A&A_GaiaDR2}
\bibinfo{author}{{Gaia Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{Gaia Data Release 2. Summary of the contents and
  survey properties}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{616}},
  \bibinfo{pages}{A1} (\bibinfo{year}{2018}).

\bibitem{2003ApJ...589L..33Y}
\bibinfo{author}{{Yu}, W.}, \bibinfo{author}{{Klein-Wolt}, M.},
  \bibinfo{author}{{Fender}, R.} \& \bibinfo{author}{{van der Klis}, M.}
\newblock \bibinfo{title}{{Hard X-Ray Flares Preceding Soft X-Ray Outbursts in
  Aquila X-1: A Link between Neutron Star and Black Hole State Transitions}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{589}},
  \bibinfo{pages}{L33--L36} (\bibinfo{year}{2003}).

\end{thebibliography}

